Self-consistent bounds method for dissipative PDEs

We discuss the method of self-consistent bounds for dissipative PDEs with periodic boundary conditions. We prove convergence theorems for a class of dissipative PDEs, which constitute a theoretical basis of a general framework for construction of an algorithm that computes bounds for the solutions of the underlying PDE and its dependence on initial conditions. We also show, that the classical examples of parabolic PDEs including Kuramoto-Sivashinsky equation and the Navier-Stokes on the torus fit into this framework.

==> bndOneStep.tex <==


\section{The existence of uniform bounds for all Ga\-ler\-kin
  projections for short time steps}
\label{sec:gendiss}




\subsection{A time step - $C^0$}
\label{subsec:C0-timestep}

The goal of this section is to twofold: \newline
1) in the context of Theorem~\ref{thm:limitLN} to show that it is relatively straightforward to construct set satisfying  (\ref{eq:appriori-bnds}), i.e. apriori bounds for a time step for all Galerkin projections,  and all our conditions C1,C2,C3,C4,D \newline
2) outline the basic principle of algorithm for rigorous integration equation (\ref{eq:feqLN}).


	
	
\begin{theorem}  \cite[Thm. 3.7]{ZKS3}
\label{thm:selfexists} Consider (\ref{eq:fugenpde}). Assume that
conditions (\ref{eq:lambdak}), (\ref{eq:lambdak2}) and
(\ref{eq:p>r}) hold. Let $s_0=p+d+1$


Let  $Z \oplus T_0$ form self-consistent bounds for
(\ref{eq:fugenpde}), such that for some $C_0$ and $s \geq s_0$
holds
\begin{equation*}
  |T_{0,k}| \leq \frac{C_0}{|k|^{s}}, \qquad |k| >m,\: k \in I, \:
  s> s_0
\end{equation*}

Then there exist $h >0$, $W \oplus T_1$ - self-consistent bounds
for (\ref{eq:fugenpde}) and $L >0$, such that for all $l >L$ and
$u \in  P_l(Z \oplus T_0)$
\begin{equation*}
  \varphi^l([0,h],u) \subset W \oplus T_1.
\end{equation*}
and
\begin{equation*}
  |T_{1,k}| \leq \frac{C_1}{|k|^{s}}, \qquad |k|>m, k \in I.
\end{equation*}
\end{theorem}
\textbf{Proof:} Let $W \subset X_m$, be  a compact set, such that
$Z \subset \inte_{X_m} W$.

By eventually increasing $C_0$ we can assume that
\begin{equation*}
  |u_k| \leq \frac{C_0}{|k|^{s}}, \qquad \mbox{for all  $u \in W \oplus T_0$ and $k \in
  I$}.
\end{equation*}

We set $C_1=2C_0$ and define the tail $T_1$  by
\begin{equation*}
   T_1=\Pi_{|k|>m, k \in I} \overline{B}\left(0,\frac{C_1}{|k|^s}\right).
\end{equation*}

\textbf{PZ:  tu powinnismy uzyc lemat o izolacji Lemma~\ref{lem:iso-mainVar}  zamiast tego co ponizej - poczatek}


From Lemma~\ref{lem:Dgen} it follows that there exists
$D=D(C_1,s)$, such that
\begin{equation*}
  |N_k(u)| < \frac{D}{|k|^{s - r}}, \quad \mbox{for all $u$, such that $|u_k| \leq \frac{C_1}{|k|^s}$}
\end{equation*}

Let $u \in W \oplus T_1$ and $|u_{k_0}|=\frac{C_1}{|k_0|^{s}}$ for
some $|k_0| > K_-$.
\begin{eqnarray}
  \frac{1}{2}\frac{d}{dt}(u_{k_0}|u_{k_0}) < -\alpha_0 |k_0|^p |u_{k_0}|^2 + |u_{k_0}| |N_{k_0}(u)| \leq  \nonumber\\
   \left(- \alpha_0 C_1 |k_0|^{p-s} + D |k_0|^{r -s}\right) |u_{k_0}|, \nonumber \\
  \frac{d|u_{k_0}|^2}{dt}< 0, \qquad |k_0|> L,  \label{eq:farentry}
\end{eqnarray}
for $L$ sufficiently large.
\textbf{dotad}

Consider now the differential inclusion
\begin{equation}
  x' \in P_LF(x) + \Delta, \qquad x \in X_L, \Delta \subset X_L  \label{eq:galediffincl}
\end{equation}
where the set $\Delta$ represents the Galerkin projection errors
on $W \oplus T_1$ and is given by
\begin{equation*}
  \Delta=\{ P_LF(u) - P_L F(P_Lu) \: | \: u \in W \oplus T_1  \}.
\end{equation*}
As it was mentioned in the introduction, by a solution of
differential inclusion (\ref{eq:galediffincl}) we will understand
any $C^1$ function $x:[0,t_m] \to X_L$ satisfying condition
(\ref{eq:galediffincl}).



It is easy to see that there exists $h >0$, such that if
$x:[0,t_m]\to X_L$, where $t_m \leq h$, is a  solution of
(\ref{eq:galediffincl}) and $x(0) \in P_L(Z \oplus T(0)))$, then
\begin{equation}
x(t)  \in \inte_{X_L} P_L (W \oplus T_1), \qquad t \in [0,h].
\label{eq:dinclencl}
\end{equation}
Namely, it is enough to take $h>0$ satisfying the following
condition
\begin{equation*}
   h \cdot \left(\max_{u \in W \oplus T_1 \in } |P_LF(u)| + \max_{\delta \in \Delta}
   |\delta|\right) < \dist(P_L(Z \oplus T_0),\partial_{X_L} P_L(W\oplus
   T_1)).
\end{equation*}

Let $l > L$ and let $u:[0,t_1) \to X_l$ be a solution of
\begin{equation*}
  u'=P_lF(u), \qquad u(0) = u_0 \in P_l(X \oplus T_0).
\end{equation*}
By changing the vector field in the complement of  $P_l (W \oplus
T_1)$ we can assume that $t_1=\infty$.

Let
\begin{equation*}
  t_m=\sup\{ t >0 \: | \: u([0,t]) \subset P_l (W \oplus
T_1)\}.
\end{equation*}
Obviously $t_m >0$. It is enough to prove that $t_m \geq h$.
Observe that for $t \in [0,t_m]$ $P_Lu(t)$ is a solution of
(\ref{eq:galediffincl}), hence from (\ref{eq:dinclencl}) we obtain
\begin{equation*}
  P_L u([0,t_m])  \subset \inte_{X_L} P_L (W \oplus T_1).
\end{equation*}
From (\ref{eq:farentry}) it follows immediately that
\begin{equation*}
  Q_L u([0,t_m]) \subset \inte_{Y_l} P_lQ_L(W \oplus T_1).
\end{equation*}
Hence
\begin{equation*}
   u(t_m) \in \inte_{X_l} P_l(W \oplus T_1).
\end{equation*}
From above condition and the continuity of $u$ it follows that for
some $\delta >0$ holds
\begin{equation*}
   u(t_m+t') \in \inte_{X_l} P_l(W \oplus T_1), \qquad t'\in [0,\delta]
\end{equation*}
hence $t_m=h$.
 \qed


\subsection{A time step for variational equation}

As in the previous section we have two goals
\begin{itemize}
\item in the context of Theorem~\ref{thm:c1conver} , we construct sets $W_{C_j}$ satisfying condition (\ref{eq:var-a-priori-bnds}) and
containing $e_j$, i.e. we construct a priori bounds for all columns with the same time step
\item to propose the method of bounding all columns of $V(t,x)$ using a finite representation. This is followed by outlining basic principle of the algorithm for integration
  of system (\ref{eq:sysVar1},\ref{eq:sysVar2}).
\end{itemize}

\subsubsection{A priori bound for all columns}

In the context of Theorem~\ref{thm:c1conver}  we assume that we have set $Z\subset W$ satisfying its assumptions. Additionally we assume that $W \subset W_P(C,s)$.
We want to find  a family of sets $\{W_{C_j}\}_{j \in \mathbb{Z}_+}$ contained in $H$, such that for each $j \in \mathbb{Z}_+$ condition \VL is satisfied on $W \times W_{C_j}$ and
for any $n >j$ the solution of the variational problem (\ref{eq:sysVar1}--\ref{eq:sysVar2}) with initial conditions $x^n(0) \in Z$ and $C^n(0)=e_j$ satisfies
\begin{equation}
  C^n(t) \in W_{C_j}, \quad t \in [0,T]. \label{eq:step-var-a-priori-bnds}
\end{equation}
Let $l$ be a constant from condition \textbf{D} for $W$.

From Lemma~\ref{lem:estmLogN} \textbf{PZ: moze inny lemat?} it follows that for all $j$ and any $n>j$ solution of the variational problem (\ref{eq:sysVar1}--\ref{eq:sysVar2}) with initial conditions $x^n(0) \in Z$ and $C^n(0)=e_j$ satisfies
\begin{equation}
  \|C^n(t)\| \leq e^{lt}, \quad t \in [0,T]. \label{eq:ln-estm-var}
\end{equation}

Let $L=L(C,s,d)$ from the isolation property in Lemma~\ref{lem:iso-VarVar}.


Let $C_{V,j}$ be such that
\begin{equation}
  C_{V,j} > |j|^s  \label{eq:CVj}
\end{equation}
and the following condition hold 
\begin{equation}
\mbox{if} \quad  y \in H \, \exists k \,  |k|\leq L \quad |y_k|=\frac{C_{V,j}}{|k|^s}, \quad \mbox{then} \, \|y\| > \max(1,e^{lT}).  \label{eq:iso-cond-v}
\end{equation}
Existence of such $C_{V,j}$ is an easy consequence of \NC5.



\begin{lemma}
\label{lem:WCj-exist}
  $W_{C_j}=\overline{B}(0,\max(1,e^{lT})) \cap W_P(C_{V,j},s)$ satisfies (\ref{eq:step-var-a-priori-bnds}) and $e_j \in W_{C_j}$.
\end{lemma}
\textbf{Proof:}
Observe that (\ref{eq:CVj}) implies that $e_j \in W_{C_j}$.

To prove (\ref{eq:step-var-a-priori-bnds}) observe that $C^n(t) \in \overline{B}(0,\max(1,e^{lT})) $ for $t \in [0,T]$. Therefore for $C^n(t)$ to exit from
$W_{C_j}$ we need that for some $t \in [0,T]$ holds $|y_k(t)|=\frac{C_{V,j}}{|k|^s}$ for some $|k| \leq n$.  Let $t_e$ be an infinum of such $t$.

We have for $t \in [0,t_e]$ that $C^n(t) \in W_{C_j}$ and  $|y_k(t_e)|=\frac{C_{V,j}}{|k|^s}$ for some $|k| \leq n$.  From condition (\ref{eq:iso-cond-v})
it follows that $|k|>L$, but for such $k$ the isolation property implies that $|y_k(t_e)|<\frac{C_{V,j}}{|k|^s}$. This is a contradiction.

\qed


\subsubsection{One step for variational system with finite representation}

In principle Theorem~\ref{thm:c1conver} and sets $W_{C_j}$ as constructed in Lemma~\ref{lem:WCj-exist} alow us to make one time step for system (\ref{eq:sysVar1}--\ref{eq:sysVar2}) provided
we can do such time step for  (\ref{eq:sysVar1}). However this is not satisfying from the computer assisted proofs point of view, as we would need an infinite number of columns to
be integrated one by one. 

To overcome this problem 
we consider block decomposition as defined in Section~\ref{subsec:lmgssblk-decmp}.

In principle any $\mathcal C^0$ algorithm can be applied to compute finite number of columns $V_{*j}(t)$ for $j=1,\dots,m$. The remaining block of infinite number of columns will be bounded uniformly by an operator norm.

For our further considerations it is convenient to split the phase space into $u=(x,y)$, where $x\in \mathbb{R}^m=:X$, $y$ is in the complementary subspace $Y$ and use the notation
\begin{equation*}
  V(t) =\left[\begin{array}{cc}
                  V_{xx}(t) & V_{xy}(t) \\
                   V_{yx}(t) & V_{yy}(t)
               \end{array}
        \right].
\end{equation*}
We  demand that $H=X \oplus Y$ is \gss and norms on $X$ and $Y$ are inherited from $H$.

In what follows we assume that the blocks $V_{xx}(t)$ and $V_{yx}(t)$ are computed using our $\mathcal C^0$ algorithm for integration of (\ref{eq:fueq}) .
Therefore for $V_{ij}(t)$ for $i,j=1,\dots,m$ are given coordinate-wise interval bounds and for  $V_{ij}$ with $j \leq m$ and $i>m$ we will have uniform bounds decaying with $i \to \infty$ depending on some constants computed by the algorithm, just like in $\mathcal C^0$ computation of $u(t)$.

Blocks  $V_{xy}$ and $V_{yy}$  will be represented in our algorithm by bounds of their operator norms. These norms will be controlled by means of the estimates from Theorem~\ref{thm:lineqestm-inf}.






==> conver-var.tex <==
\section{Proof of Theorem \ref{thm:c1conver}.}
\label{sec:c1converproof}




We extend $V^n:[0,T] \times P_n(Z)  \to \mbox{Lin}(H_n,H_n)$ to $V^n:[0,T] \times Z \to \mbox{Lin}(H,H)$ by setting $V^n(t,x)=V^n(t,P_nx)$.


We apply Theorem~\ref{thm:limitLN}  to variational system for $j$-th column. From \VL it follows that all its assumptions are satisfied
for system (\ref{eq:sysVarH}) with $Z_V=Z \times \{e_j\}$ and $W_V=W \times W_{C_j}$ with $l=A$ from condition \VL{}-D.  Therefore
there exists a family of continuous functions
$V_{\ast j}:[0,\infty)\times Z \to H$ for $j \in \mathbb{Z}_+$, such that for each $j$ the functions
$V^{n}_{\ast j}$ converge to $V_{\ast j}$ uniformly on $[0,T] \times Z$.

Moreover, $(z(t),V_{\ast j}(t,z))$ satisfies variational equation (\ref{eq:sysVarH}).


Now we  prove (\ref{eq:intpar}) and (\ref{eq:dfiduj=Vij}).

Let us fix $t \in [0,T]$.

For any  $n$ we have
\begin{equation}
  \varphi^n(t,P_n x) - \varphi^n(t,P_n y) =   \int^1_0 V^n(t,P_n y+s(P_n x- P_n y))ds \cdot P_n(x-y)
\end{equation}

We will pass to the limit $n \to \infty$ in above equation. The limit of l.h.s.
is settled by Theorem \ref{thm:limitLN}.


Now we consider the r.h.s.  We will use Theorem~\ref{thm:Vn-weak-lim} to pass to the limit $n \to \infty$.

From condition \textbf{D}  and Lemma~\ref{lem:estmLogN} it follows that for all $n$, $x,y \in Z$ and $t \in [0,T]$
\begin{equation*}
  \|\varphi^n(t,x) - \varphi^n(t,y)\| \leq e^{lt} \|x-y\|,
\end{equation*}
hence
\begin{equation}
  \|V^n(t,x)\| \leq e^{lt}, \qquad \forall n, (t,x) \in [0,T] \times Z. \label{eq:VnlogN}
\end{equation}


Let $\overline{V}^n(t,[x,y])=\int^1_0 V^n(t,y+s(x- y))ds$.  From (\ref{eq:VnlogN})  we have for $x,y \in Z$
\begin{equation}
  \|V^n(t,x)\| \leq e^{lt}, \quad   \|\overline{V}^n(t,[x,y])\| \leq e^{lt}.
\end{equation}
From convexity of $W_{C_j}$ it follows that for all $j$ holds
\begin{equation}
  V_{\ast j}^n(t,x),\overline{V}^n(t,[x,y])_{\ast j} \in W_{C_j}.
\end{equation}
Since for all $i,j$  $V^n_{ij}(t,\cdot)$ are continuous on $Z$ and converge uniformly to $V_{ij}(t,\cdot)$, therefore
\begin{equation}
  \int^1_0 V^n_{ij}(t,y+s(x- y))ds \to \int^1_0 V_{ij}(t,y+s(x- y))ds.
\end{equation}
Now we use Theorem~\ref{thm:Vn-weak-lim} to conclude that $V \in \mbox{Lin}(H,H)$, $\int^1_0 V(t,y+s(x- y))ds \in \mbox{Lin}(H,H)$ and
\begin{equation}
  \lim_{n \to \infty} \int^1_0 V^n(t,y+s(x- y))ds \cdot (x-y) = \int^1_0 V(t,y+s(x- y))ds \cdot (x-y).
\end{equation}

Observe that from  formula (\ref{eq:intpar}) we obtain
 (\ref{eq:dfiduj=Vij}). Indeed, we have
\begin{eqnarray*}
  \varphi(t,x+he_j) -  \varphi(t,x) = h \int_0^1 V_{j}(t,x+she_j)ds \cdot e_j \\
  = h  V(t,x)e_j + h \int_0^1 \left( V(t,x+she_j)e_j - V(t,x)e_j \right)ds\\
  = h  V_{\ast j}(t,x) + h \int_0^1 \left( V_{\ast j}(t,x+she_j) - V_{\ast j}(t,x) \right)ds
\end{eqnarray*}
and the result follows from continuity of $V_{\ast j}(t,\cdot)$.

It remains to prove that for every $a \in H$ the map $[0,T] \times Z \ni (t,z) \mapsto V(t,z)a \in H$ is continuous.

We know that for every $j$ the map $(t,x) \mapsto V_{\ast j}(t,z)$ is continuous.

Let $(t_1,z_1), (t_2,z_2) \in [0,T] \times Z$. Then  for any $n$ holds
\begin{eqnarray*}
  \| V(t_1,z_1)a - V(t_2,z_2)a \| \leq \| V(t_1,z_1)P_n a - V(t_2,z_2)P_n a \| \\
   +  \| V(t_1,z_1)(I-P_n) a \| + \| V(t_2,z_2)(I-P_n) a \| \leq  \\
       \sum_{j \in J_n} \|V(t_1,z_1)_{\ast j} - V(t_2,z_2)_{\ast j}\| \cdot |a_j| + (e^{t_1 l} + e^{t_2 l}) \|(I-P_n)a\|
\end{eqnarray*}
For a given $\epsilon>0$ we take $n$ so large that $ \|(I-P_n)a\|e^{\max(0,l)T} < \epsilon/2$. We fix such $n$. Then from the continuity of $V_{\ast j}$ for $j\in J_n$
we can make the sum less that $\epsilon/2$ when $(t_2,z_2) \to (t_1,z_1)$. This finishes the proof.

\qed








==> converC0.tex <==
\section{Convergence of Galerkin projections}
\label{sec:limitlogn}


We will here use  the notations introduced in Section
\ref{sec:c1-conver}.
The goal of this section is to present the proof of the
existence of the  limit of Galerkin projections of problem (\ref{eq:feqLN}).


\noindent
\textbf{Proof of Theorem~\ref{thm:limitLN}:}
Let
\begin{displaymath}
\delta_n= \max_{x \in W} \|P_n(F(x)) - P_n(F(P_n x))\|.
\end{displaymath}
 Obviously $\delta_n \to 0$ for $n \to \infty $, because $F \circ
 P_n$ converges uniformly to $F$ on $W$ - this follows immediately from \textbf{C2} and \textbf{C3}.

Let
\begin{equation}
   l_n=\sup_{x \in P_n W}\mu\left(D P_n F_{|H_n} (x) \right).
\end{equation}

From  assumption {\bf D}, it follows that  $l_n$ are uniformly
bounded, namely
\begin{equation}
  l_n \leq l, \quad \mbox{for all $n$}.
\end{equation}

Let us take $k \geq n$. Let $x_n:[0,T] \to P_nW$ and $x_k:[0,T]
\to P_k W$ be the solutions of $n$- and $k$-dimensional
projections of (\ref{eq:feqLN}) with initial conditions in $Z$, respectively.

Observe that for $t \in [0,T]$ holds
\begin{eqnarray*}
  (P_n x_k(t))'&=&P_n F(x_k(t))\\
  &=&P_n F(P_nx_k(t)) + (P_n F(x_k(t)) - P_n F(P_nx_k(t)) ),
\end{eqnarray*}
hence we can treat $y(t)=P_n x_k(t)$ as "perturbed solution" of $n$-th Galerkin projection of (\ref{eq:feqLN}) with the size of perturbation
 estimated by $\delta_n$ as follows
\begin{eqnarray*}
  \|P_n F(x_k(t)) - P_n F(P_nx_k(t))\| &\leq& \delta_n.
\end{eqnarray*}
 From Lemma \ref{lem:estmLogN} it
follows immediately that
\begin{equation}
  \|x_n(t) - P_n(x_k(t))\| \leq e^{lt}\|x_n(0) - P_nx_k(0)\| + \delta_n \frac{e^{lt} - 1}{l}
  \label{eq:estmdiffg}
\end{equation}

To prove the uniform convergence of $\{x_n\}$ starting from the
same initial condition,  observe that
\begin{eqnarray*}
 \|x_n(t) - x_k(t)\| \leq  \|x_n(t) - P_n(x_k(t))\| + \|(I-P_n) x_k(t)\| \leq \\
    \delta_n \frac{e^{lt} - 1}{l} + \|(I-P_n) x_k(t)\| \leq
     \delta_n \frac{e^{lT} - 1}{l} + \|(I-P_n)W\|.
\end{eqnarray*}
Since by Lemma~\ref{lem:compt-gss} $\|(I-P_n)W\| \to 0$ for $n \to \infty$ we see
 that $\{x_n\}$ is a Cauchy sequence in $\mathcal{C}([0,T],H)$, hence it converges uniformly to $x^*:[0,T]\to W$.

Since $x_n(t)$ satisfies an integral equation
\begin{equation*}
  x_n(t)=x_n(0) + \int_0^t P_n F(x_n(s))ds,
\end{equation*}
then from the uniform continuity of $F$ on $W$ it follows that after passing to the limit $n \to \infty$ that
\begin{equation*}
  x^*(t)=x^*(0) + \int_0^t  F(x^*(s))ds,
\end{equation*}
which implies that $x^*$ is a solution of (\ref{eq:feqLN}).


\textbf{Uniqueness.} Let $x:[0,T] \to W$ be a solution of
(\ref{eq:feqLN}) with the initial condition $x(0)=x_0$. We will
show that $x_n $ converge to $x$. We apply Lemma
\ref{lem:estmLogN} to $n$-dimensional projection and the function
$P_n x(t)$. We obtain
\begin{equation}
  \|x_n(t) - P_n(x(t))\| \leq  \delta_n \frac{e^{lt} - 1}{l}.
\end{equation}
Since the tail $\|(I-P_n)x(t)\| \leq \|(I-P_n)W\|$ is by Lemma~\ref{lem:compt-gss} uniformly converging to zero as $n
\to \infty $, we see that $x_n \to x$ uniformly.


\textbf{Lipschitz constant on $W$}. From Lemma~\ref{lem:estmLogN}
applied to $n$-dimensional Galerkin projection for different
initial conditions (we denote the functions by $x_n$ and $y_n$ and
the initial conditions $x_0$ and $y_0$), we obtain
\begin{equation}
  \|x_n(t) - y_n(t)\| \leq e^{lt}\|P_n x_0 - P_n y_0\|.
  \label{eq:diffnlip}
\end{equation}
Let $x_n \to x$ and $y_n \to y$. Then passing to the limit in
(\ref{eq:diffnlip}) gives
\begin{equation}
  \ |x(t) - y(t)\| \leq e^{lt}\|x_0 - y_0\|.
\end{equation}

Assertion 4 follows easily from the previous ones. \qed


==> decayVar.tex <==
\section{Decay in rows and columns for variational matrix}


 Assume that we have a solution $x(t)$ for $t \in [0,T]$, contained in self-consistent polynomial bounds $W$ (i.e. all convergence conditions are satisfied) such that
 \begin{equation*}
   |x_k| \leq \frac{\tilde{C}}{|k|^s}
 \end{equation*}
 with $s$ sufficiently large.


Each column evolves separately. Let us fix $j_0$ - this is our column. We look at the variational equation with initial condition $v=e_{j_0}$.


\subsection{Special case}

In case when $N(u,u_x)=(P(u))_x$ (this is true for KS)
 Then the derivative of non-linear part satisfies  
 \begin{equation}
   \left|\frac{\partial N_i}{\partial x_j}(x(t))\right| \leq \frac{D_1 |i|^r}{|i-j|^s}.  \label{eq:estm-DNv}
 \end{equation}
the same is true for Navier-Stokes system \cite{Z}.


We look for the a-priori bound of the form
\begin{equation*}
  |v_i| \leq \frac{C}{|i-j_0|^s}.
\end{equation*}


The part coming from  $\sum_{j} \frac{\partial N_i}{\partial v_j} v_{j}$ is due to Lemma~\ref{lem:estmQ2} estimated as follows
\begin{eqnarray*}
  \left|\sum_{j} \frac{\partial N_i}{\partial v_j} v_{j}  \right| \leq \sum_{j} \frac{D_1 |i|^r}{|i-j|^s} \frac{C}{|j-j_0|^s}  \leq \frac{|i|^rD_1 C C_2(d,s)}{|i-j_0|^s}
\end{eqnarray*}
For the isolation condition it is enough to have
\begin{eqnarray*}
   -\lambda_i \frac{C}{|i-j_0|^s} > \frac{|i|^rD_1 C C_2(d,s)}{|i-j_0|^s}
\end{eqnarray*}
Using (\ref{eq:lambdak},\ref{eq:lambdak2}) we see that it is enough to have
\begin{equation*}
  \alpha_0 |i|^p > |i|^r D_1 C_2(d,s)
\end{equation*}
which holds if 
\begin{equation*}
  |i| > \left(\frac{ D_1 C_2(d,s)}{\alpha_0} \right)^{\frac{1}{p-r}}.
\end{equation*}
Observe that $C$ is not involved in this condition.  We can take $C=1$ to include the initial condition.  Therefore we proved
\begin{lemma}
  Assume that (\ref{eq:estm-DNv}) holds for $t \in [0,T]$ and
  \begin{equation*}
  |i| > K_r=\left(\frac{ D_1 C_2(d,s)}{\alpha_0} \right)^{\frac{1}{p-r}}.
  \end{equation*}
  Then
  \begin{equation*}
      |V_{i,j_0}(t)| \leq \frac{1}{|i-j_0|^s}.
  \end{equation*}
\end{lemma}
Observe that the above lemma gives us decay in rows with $i > K_r$ of the desired form and also decay in all columns.

What is not controlled is the behavior of first coordinates in each column, with $i \leq K_r$. 

==> isolation_old.tex <==

\subsection{Isolation property}

\textbf{PZ: byc moze dac to do wstepu}


To illustrate the \emph{isolation property}
let us consider a class of dissipative PDEs of the following form
\begin{equation}
  u_t = L u + N\left(u,Du,\dots,D^ru\right), \label{eq:genpde}
\end{equation}
where $u \in \mathbb{R}^n$,  $x \in \mathbb{T}^d=\left(\mathbb{R}\mod 2\pi\right)^d$, $L$ is a linear operator, $N$ is a
polynomial and by $D^s u$ we denote $s^{\text{th}}$ order derivative of
$u$, i.e. the collection of all spatial partial derivatives of $u$ of
order $s$. The reason to consider polynomial and not more general functions $N$ is technical --- we need to compute
the Fourier coefficients of $N\left(u,Du,\dots,D^ru\right)$. This can be achieved by taking suitable convolutions of Fourier expansions of $u$ and its spatial partial derivatives.

We require, that the operator $L$ is diagonal in the Fourier basis
$\{e^{ikx}\}_{k \in \mathbb{Z}^d}$,
\begin{equation*}
  L e^{ikx}= -\lambda_k e^{ikx},
\end{equation*}
with
\begin{eqnarray*}
 L_* |k|^p &\leq& \lambda_k \leq  L^* |k|^p, \qquad \text{for all $|k| > K$ and  $K,L_*,L^* \geq 0$}, \\
    p &>& r.
\end{eqnarray*}

If the solutions are sufficiently smooth, the problem (\ref{eq:genpde}) can be written as an infinite ladder of ordinary differential equations for the Fourier
coefficients in $u(t,x)=\sum_{k \in \mathbb{Z}^d} u_k(t) e^{i kx}$, as follows
\begin{equation}
  \frac{d u_k}{dt} = F_k(u)=-\lambda_k u_k + N_k\left(\{u_j\}_{j \in \mathbb{Z}^d}\right), \qquad \mbox{for all
  $k \in \mathbb{Z}^d$}. \label{eq:fueq}
\end{equation}



The crucial fact, which makes our approach to the rigorous integration of (\ref{eq:fueq})  possible is the \emph{isolation property}, which reads:

\emph{Let}
\begin{equation*}
   W=\left\{ \{u_k\}_{k \in \mathbb{Z}^d}\,|\,  |u_k| \leq \frac{C}{|k|^s q^{|k|}}\right\}
\end{equation*}
\emph{where $q\geq 1$, $C>0$, $s>0$. \\
Then there  exists $K>0$, such that for $|k| > K$ there holds}
\begin{equation*}
 \mbox{if} \quad u \in W, \ |u_k|=\frac{C}{|k|^s q^{|k|}}, \qquad \mbox{then} \qquad  u_k \cdot F_k(u) <0.
\end{equation*}

For the proof of  the above fact see Theorem 3.1 and its proof in \cite{ZKS3}, where the case with $q=1$ was treated.

Projection of the set $W$ onto $k^{\mathrm{th}}$ mode is a closed disc (or interval) centred at zero and of radius
$r_k =\frac{C}{|k|^s q^{|k|}}$. Geometrically the isolation property means that if $|u_k|=r_k$ for some $k> K$ then the $k$-th component of the vector field is pointing inwards the set. As a consequence, the only way a trajectory may leave the set $W$ forward in time is by increasing some of leading modes $|u_k|$, $k\leq K$ above the threshold $r_k$. However, one has to be careful with what "inwards" means in the above statement because $W$ has empty interior as a compact subset in infinite dimensional space.


This property is used   in  our approach to obtain a priori bounds for $u_k(h)$ for small $h>0$ and $|k|>K$, while the leading modes $u_k$ for $|k| \leq K$ are computed using  tools for rigorous integration of ODEs \cite{CAPDREVIEW,Lo,NJP} based on the interval arithmetics \cite{Mo}, i.e. to obtain set $W$ as in Theorem~\ref{thm:limitLN}. Moreover, from the point of view of topological method, the isolation property is of crucial importance as it shows that on the tail we have the entry behaviour, which enable us to apply the finite dimensional tools from the dynamics.


In this work we use sets of the type described above with $s=0$ and $q>1$. The isolation property for KS equation on such sets is established in \cite[Rem. 19]{WZ}.


==> lognorm.tex <==
\section{Logarithmic norms}
\label{sec:lognorm}


\begin{definition} \cite{D58,L58}
\label{def:lognorm}
 Let $\| \cdot \|$ denote a vector norm on $\mathbb{R}^n$  as
well as its subordinate operator norm on $\mathbb{R}^{n
\times n}$. The \emph{logarithmic
norm} of operator $A$ is
\begin{equation}
  \mu(A)=\lim_{h \to 0^+} \frac{\|\mathrm{Id} + hA \| - 1}{h} \label{eq:lnormdef}
\end{equation}
\end{definition}
For the properties and the use of the logarithmic norm see \cite{KZ} and the literature given there.



Consider the differential equation
\begin{equation}
  x'=f(x), \quad \mbox{$f \in C^1$}. \label{eq:odelogn}
\end{equation}
Let $\varphi(t,x_0)$  denote the solution of equation
(\ref{eq:odelogn}) with the initial condition $x(0)=x_0$. By $\|x
\|$ we denote a fixed arbitrary norm in $\mathbb{R}^n$.


From Lemma~\ref{lem:boundOnVariationalLinEq} one can easily derive the following result.
\begin{lemma}
\label{lem:estmLogN} Let $y:[0,T] \to \mathbb{R}^n$ be a piecewise
$C^1$ function and $\varphi(\cdot,x_0)$ be defined for $t \in
[0,T]$. Suppose that $Z$ is a convex set such that   the following
estimates hold:
\begin{eqnarray*}
  y([0,T]), \varphi([0,T], x_0) \in Z  \\
  \mu\left(\frac{\partial f}{\partial x}(\eta)\right) \leq l,\quad \mbox{ for $\eta \in Z$} \\
  \left\| \frac{dy}{dt}(t) - f(y(t)) \right\| \leq \delta.
\end{eqnarray*}
Then for $0 \leq t \leq T$ there is
\begin{displaymath}
 \| \varphi(t,x_0) - y(t)  \| \leq e^{lt}  \|y(0) - x_0 \| + \delta \frac{e^{lt} -1}{l},\quad \mbox{if $l \neq 0$}.
\end{displaymath}
For $l=0$, there is
\begin{displaymath}
 \| \varphi(t,x_0) - y(t)  \| \leq  \|y(0) - x_0 \| + \delta t.
\end{displaymath}
\end{lemma}


In the paper we frequently use norm  $\|x\|_{\infty}=\max_{i=1,\dots,n} |x_i|$ on $\mathbb{R}^n$.  
\begin{lemma}
\label{lem:logNormMax}
  Let $A \in \mathbb{R}^{n \times  n}$, then the logarithmic norm of $A$ induced by norm $\| \cdot \|_\infty$ is given by
  \begin{equation}
    \mu(A)=\max_{i=1,\dots,n} \left( A_ii + \sum_{k=1 , k\neq i}^n |A_{ik}| \right). \label{eq:logNormMax}
  \end{equation}
 \end{lemma}

